Individually Addressable and Spectrally Programmable Artificial Atoms in Silicon Photonics

Artificial atoms in solids have emerged as leading systems for quantum information processing tasks such as quantum networking, sensing, and computing. A central goal is to develop platforms for precise and scalable control of individually addressable artificial atoms that feature efficient optical interfaces. Color centers in silicon, such as the recently-isolated carbon-related 'G-center', exhibit emission directly into the telecommunications O-band and can leverage the maturity of silicon-on-insulator (SOI) photonics. Here, we demonstrate the generation, individual addressing, and spectral trimming of G-center artificial atoms in a SOI photonic integrated circuit (PIC) platform. Focusing on the neutral charge state emission at 1278nm, we observe waveguide-coupled single photon emission with an exceptionally narrow inhomogeneous distribution with standard deviation of 1.1nm, an excited state lifetime of 8.3$\pm$0.7ns, and no degradation after months of operation. In addition, we introduce a technique for optical trimming of spectral transitions up to 300 pm (55 GHz) and local deactivation of single artificial atoms. This non-volatile "spectral programming" enables the alignment of quantum emitters into 25 GHz telecommunication grid channels. Our demonstration opens the path to quantum information processing based on implantable artificial atoms in very large scale integrated (VLSI) photonics.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        # FOR PDFLATEX
        system( "latexmk -cd -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk -cd \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -cd -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -cd -lualatex \"$_[0]\"" );
   }
}
